Identification of Parameters for Large-scale Kinetic Models

Inverse problem for the identification of the parameters for large-scale systems of nonlinear ordinary differential equations (ODEs) arising in systems biology is analyzed. In a recent paper in \textit{Mathematical Biosciences, 305(2018), 133-145}, the authors implemented the numerical method suggested by one of the authors in \textit{J. Optim. Theory Appl., 85, 3(1995), 509-526} for identification of parameters in moderate scale models of systems biology. This method combines Pontryagin optimization or Bellman's quasilinearization with sensitivity analysis and Tikhonov regularization. We suggest modification of the method by embedding a method of staggered corrector for sensitivity analysis and by enhancing multi-objective optimization which enables application of the method to large-scale models with practically non-identifiable parameters based on multiple data sets, possibly with partial and noisy measurements. We apply the modified method to a benchmark model of a three-step pathway modeled by 8 nonlinear ODEs with 36 unknown parameters and two control input parameters. The numerical results demonstrate geometric convergence with a minimum of five data sets and with minimum measurements per data set. Software package \textit{qlopt} is developed and posted in GitHub. MATLAB package AMIGO2 is used to demonstrate advantage of \textit{qlopt} over most popular methods/software such as \textit{lsqnonlin}, \textit{fmincon} and \textit{nl2sol}.

==> figs/rp_numOfDataPntsTable.tex <==
\begin{table}
\centering
\sisetup{
    round-mode = places,
    round-precision = 7,
    %table-number-alignment = center,
}
\begin{tabular}{SS}
		\toprule
		{\# of data point} & {$||\mathbf{x} - \mathbf{x}_{N}||$} \\ \midrule
 2001 & 0.01899218 \\
 1001 & 0.01899207  \\
 501 & 0.01898387  \\
 201 & 0.01896577  \\
 101 & 0.0189798  \\
 51 & 0.02517813  \\
 41 & 0.03953422  \\
 34 & 0.06170568  \\
 26 & 0.1073747  \\
 21 & 0.2053257
\\
		\bottomrule
	\end{tabular}
\caption{Table of the number of data points vs.
$||\mathbf{x} - \mathbf{x}_{N}||$
for the repressilator model. The parameters were
$\mathbf{u}_0 =\allowbreak  (175,.5,1,.5,\allowbreak .5,175,\allowbreak .5,1,.5,.5,175,\allowbreak .5,1,\allowbreak .5,.5)$,
	$\mathbf{u}^* =\allowbreak  (250,.4,3,\allowbreak .4,.4,250,\allowbreak .4,3,.4,.4,250,\allowbreak .4,3,\allowbreak .4,.4)$,
	$\mathbf{u} =\allowbreak  (216,.216,2,\allowbreak .2,0.2,216,\allowbreak .216,2,.2,.2,216,\allowbreak .216,2,\allowbreak .2,.2)$,
	$\mathbf{x}_0 =\allowbreak  (5,1,10,\allowbreak 1,15,1)$,
	$\alpha = 0.00001$,
	time interval $[0,10]$
and respective tolerances were set at \(\num{1E-7}\).}
\label{tab:rp_num_data}
\end{table}


==> latexmkrc <==
$pdflatex="pdflatex --shell-escape -enable-write18 --synctex=1 -interaction=nonstopmode %O %S";

# $cwd = cwd();
# $pdf_previewer = 'osascript -e "set theFile to POSIX file \"%S\" as alias" -e "set thePath to POSIX path of theFile" -e "tell application \"Skim\"" -e "open theFile" -e "end tell"';
# $pdf_update_method = 4;
# $pdf_update_command = '/usr/bin/osascript -e "set theFile to POSIX file \"%S\" as alias" -e "set thePath to POSIX path of theFile" -e "tell application \"Skim\"" -e "  set theDocs to get documents whose path is thePath" -e "  try" -e "    if (count of theDocs) > 0 then revert theDocs" -e "  end try" -e "  open theFile" -e "end tell"';

# $pdf_previewer =~ s#pwd#$cwd#
# $pdf_update_command =~ s#pwd#$cwd#

# add_cus_dep('gnuplot', 'table', 0, 'gnuplot_sub');
# sub gnuplot_sub {
# 	system( "gnuplot \"$_[0].gnuplot\"" )
# }


==> makefile <==
PWD:=$(shell pwd)
MAINFILE=main

export CHKTEXARGS=-wall -n 6 -n 3 -n 22 -n 36 -n 30
export CHKTEX=chktex $(CHKTEXARGS)

export ASPELLPWS="$(PWD)/.aspell.en.pws"
export ASPELLCONF="$(PWD)/aspell.conf"
export ASPELL=aspell --personal=$(ASPELLPWS) --conf=$(ASPELLCONF) -a

export LATEXMKRC=$(PWD)/latexmkrc
export LATEX=latexmk -r "$(LATEXMKRC)" -bibtex -pdf -f

UNAME=$(shell uname -s)

SOURCES:=$(wildcard *.tex)
SOURCENAMES:=$(basename $(SOURCES))

###
# Global
###
all: $(MAINFILE).pdf

setup-basic:
	@mkdir -p input

setup-extra:
	@mkdir -p figs tables

setup-all:
	@mkdir -p input figs tables

#Generate pdf output using latexmk, so references & bib-file are run appropriately
$(MAINFILE).pdf: $(MAINFILE).tex references.bib
	$(LATEX) $<

# Remove byproducts of TeX generation
clean-%: %.tex
	-$(LATEX) -c $<

clean-all-%: %.tex
	-$(LATEX) -C $<

clean-srcs: $(addprefix clean-,$(SOURCENAMES))

clean-all-srcs: $(addprefix clean-all-,$(SOURCENAMES))
###
# Visualize output using Skim or Evince depending on platform
###
ifeq ($(UNAME), Darwin)
viz: $(MAINFILE).pdf
		/usr/bin/osascript -e "set theFile to POSIX file \"$(PWD)/$<\" as alias" -e "set thePath to POSIX path of theFile" -e "tell application \"Skim\"" -e "  set theDocs to get documents whose path is thePath" -e "  try" -e "    if (count of theDocs) > 0 then revert theDocs" -e "  end try" -e "  open theFile" -e "end tell"
endif
ifeq ($(UNAME), Linux)
viz: $(MAINFILE).pdf
		evince "$(PWD)/$<" &
endif

###
# check target: Run chktex on all files
###
check: $(addprefix check-,$(SOURCENAMES))

check-%: lint-%.out
	test ! -s $<

lint-%.out: %.tex
	$(CHKTEX) $< 2>/dev/null | tee $@

clean-check: $(addprefix clean-check-,$(SOURCENAMES))

clean-check-%: %.tex
	$(RM) lint-$*.out

###
# Run spellcheck on all files
###
spellcheck: $(addprefix spellcheck-,$(SOURCENAMES))

spellcheck-%: sp-%.out
	test `tail -n +2 $< | grep -e '^#' - | wc -l` -eq "0"

sp-%.out: %.tex
	$(ASPELL) < $< > $@

clean-spellcheck: $(addprefix clean-spellcheck-,$(SOURCENAMES))

clean-spellcheck-%: %.tex
	$(RM) sp-$*.out

# Clean up test output
clean-test: clean-spellcheck clean-check

clean-all-test:

###
# Flattening file for distribution
###
dist: $(MAINFILE).tar.gz $(MAINFILE).zip

%-flat.tex: %.tex
	latexpand $< > $@

%.zip: %-flat.tex %.pdf references.bib
	zip $@ $^

%.tar.gz: %-flat.tex %.pdf references.bib
	tar cvzf $@ $^

clean-dist-%: %.tex
	[ -e $*-flat.tex ] && $(LATEX) -C $*-flat.tex || echo "There is no $*-flat.tex"
	$(RM) $*.tar.gz

clean-dist: clean-dist-$(MAINFILE)

clean-all-dist:

###
# Automated formatting targets
###
fmt: $(addsuffix .bak,$(SOURCENAMES))

%.bak: %.tex
	latexindent -w -l $<

clean-fmt: $(addprefix clean-fmt-,$(SOURCENAMES))

clean-fmt-%: %.tex
	$(RM) $*.bak

###
# Combined clean targets
###
CLEANLIST=main fmt check srcs dist
clean: $(addprefix clean-,$(CLEANLIST))
	$(RM) -r auto

CLEANALLLIST=deps test dist srcs
clean-all: clean $(addprefix clean-all-,$(CLEANALLLIST))

###
# Print variable (see http://blog.jgc.org/2015/04/the-one-line-you-should-add-to-every.html)
###
print-%: ; @echo $*=$($*)


==> notes/scrap <==
%% This wasn't for wasn't with all parameters.
We first considered \(\alpha=\frac{1}{2}^N\), where \(N\) is equal to the
iteration and we used the extended precision library mpreal \cite{mpreal}.
This worked if initial guess was suffciently close and if each iteration was
generally improving in the right direction. This had many limitation, but it
showed us that we could reach convergence.
%% End


For the simpler model we could chose a constant \(\alpha\) term and it
would still converge, but with this larger model was more sensitive to the
choice of \(\alpha\) at each iteration.

With previous experiments showing that we needed a decreasing value of
\(\alpha\) at each iteration we considered \(\alpha\) as being directly
proportional to \(||\bf{x}-\bf{x}_{N}||\) which lead to convergence.

We later paralleled our problem with the trust region method. Both algorithms
consider solving a local problem using a low-order approximation. Since we are
solving the optimization problem with respect to the approximation, the
predictive power of the algorithms are only good for a small radius about
the point we are expanding. That leads the trust region method to institute a
constraint on the magnitude of the improving direction at each iteration. In
similar fashion we use \(\alpha\) to control the size of \(\Delta \bf{u}_N\).

We subsequently tried to a few experiments with \(\alpha\). We tried finding
\(\alpha\) on using a brute force method. We evenly divided up between
\(10^n\) to \(10^m\) where \(n<m\) on a log scale and found the \(\alpha\)
value that produces the lowest values for the objective function. Which amount
to solving a few linear algebraic expressions. We found that this helped us
with convergence but it was inconsistent or slow at times.

We also hypothesized that there was an optimal function that relates \(\alpha\)
to \(||\bf{x}-\bf{x}_{N}||\). So for several examples we considered
\(\alpha = c(||\bf{x}-\bf{x}_{N}||)^2\) where \(c \in \bf{R}\). We found that
for at least one value of \(c\) we would get relatively quick convergence and
changing \(c\) by \(\pm \epsilon\) the convergence would take longer.

We then tried combining the two methods by doing a brute force search for \(c\)
given the assumption that \(\alpha = c(||\bf{x}-\bf{x}_{N}||)^2\). This lead to
quicker convergence when the range was sufficiently wide, but it was to a solution
that was still for from the true solution. If you chose the range two small
than you ended up with the same problem where the solution plateaus for many
iterations before reaching convergence.

It seems that the underlying f


==> table/partial_tsmn_no_noise_05ds.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSS SSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{11}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 1.23025027 & 1.2259241 & 1.00068339 & 1 \\
		\(p_{2}\) & 1.25 & 0.991904973 & 1.05713945 & 0.998553559 & 1 \\
		\(p_{3}\) & 2.5 & 2.27634193 & 1.98914579 & 1.99999766 & 2 \\
		\(p_{4}\) & 1.25 & 1.09781731 & 0.941104282 & 1.00133844 & 1 \\
		\(p_{5}\) & 2.5 & 2.35004761 & 1.98814962 & 2.00003977 & 2 \\
		\(p_{6}\) & 1.25 & 1.2939431 & 1.25439347 & 0.999528688 & 1 \\
		\(p_{7}\) & 1.25 & 1.25699783 & 1.31013179 & 0.965145057 & 1 \\
		\(p_{8}\) & 1.25 & 0.998804724 & 1.02875195 & 1.03382884 & 1 \\
		\(p_{9}\) & 2.5 & 1.98025217 & 2.01945189 & 2.00029998 & 2 \\
		\(p_{10}\) & 1.25 & 0.936126615 & 0.967153831 & 0.967096083 & 1 \\
		\(p_{11}\) & 2.5 & 2.0694758 & 1.98633601 & 1.99960512 & 2 \\
		\(p_{12}\) & 1.25 & 1.24767743 & 1.19532872 & 0.993356331 & 1 \\
		\(p_{13}\) & 1.25 & 1.14772469 & 1.1371705 & 1.00171796 & 1 \\
		\(p_{14}\) & 1.25 & 1.15533329 & 1.08279726 & 0.999560023 & 1 \\
		\(p_{15}\) & 2.5 & 2.47302677 & 2.09253428 & 1.99872598 & 2 \\
		\(p_{16}\) & 1.25 & 0.93464079 & 0.922532758 & 1.0000011 & 1 \\
		\(p_{17}\) & 2.5 & 2.32847587 & 2.10929833 & 2.0009551 & 2 \\
		\(p_{18}\) & 1.25 & 1.33610962 & 1.26613545 & 1.00141698 & 1 \\
		\(p_{19}\) & 0.125 & 0.092350042 & 0.108094898 & 0.099688083 & 0.1 \\
		\(p_{20}\) & 1.25 & 1.2782545 & 1.22858068 & 0.994817736 & 1 \\
		\(p_{21}\) & 0.125 & 0.0786539872 & 0.0957655031 & 0.100012505 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0861304885 & 0.105160659 & 0.107448654 & 0.1 \\
		\(p_{23}\) & 1.25 & 1.25326958 & 1.26684705 & 1.11516421 & 1 \\
		\(p_{24}\) & 0.125 & 0.0765441878 & 0.0974033088 & 0.100054549 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.0702980408 & 0.0917373292 & 0.0998716446 & 0.1 \\
		\(p_{26}\) & 1.25 & 1.28015251 & 0.931293478 & 0.998805076 & 1 \\
		\(p_{27}\) & 0.125 & 0.0608035929 & 0.0943060809 & 0.0999670529 & 0.1 \\
		\(p_{28}\) & 1.25 & 1.0865762 & 0.999404049 & 0.999888468 & 1 \\
		\(p_{29}\) & 1.25 & 1.38986542 & 1.12243418 & 0.999517918 & 1 \\
		\(p_{30}\) & 1.25 & 1.20239065 & 1.38669205 & 0.998857164 & 1 \\
		\(p_{31}\) & 1.25 & 1.14416739 & 1.11245024 & 0.999479203 & 1 \\
		\(p_{32}\) & 1.25 & 1.24176529 & 1.18159147 & 0.99737998 & 1 \\
		\(p_{33}\) & 1.25 & 1.19900858 & 1.19294161 & 0.994904414 & 1 \\
		\(p_{34}\) & 1.25 & 1.2138487 & 1.02918911 & 1.00124206 & 1 \\
		\(p_{35}\) & 1.25 & 1.39801333 & 1.06288085 & 1.00232592 & 1 \\
		\(p_{36}\) & 1.25 & 0.881365728 & 1.02378513 & 1.00135985 & 1 \\
		$\alpha$ & & 1.37235292 & 0.469269427 & \num{3.11846273e-06} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 5 data sets, 4 out of 8 states, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points. Regularization parameter \(\alpha\) was determined using \eqref{eq:alphaformula} where \(C = 0.5\) and \(\gamma = 2\). }
\label{tab:partial_tsmn02}
\end{table}


==> table/tsmn_21_no_noise_05ds.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSS SSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{10}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 1.2468801 & 0.999211744 & 1.00116246 & 1 \\
		\(p_{2}\) & 1.25 & 0.929354096 & 0.999788621 & 1.00020968 & 1 \\
		\(p_{3}\) & 2.5 & 2.28327634 & 2.0006259 & 1.999535 & 2 \\
		\(p_{4}\) & 1.25 & 1.17855316 & 0.999606704 & 0.999982026 & 1 \\
		\(p_{5}\) & 2.5 & 2.54455663 & 1.998669 & 1.99998259 & 2 \\
		\(p_{6}\) & 1.25 & 1.2562049 & 0.999315372 & 1.00116117 & 1 \\
		\(p_{7}\) & 1.25 & 1.24491525 & 1.08624586 & 1.00215195 & 1 \\
		\(p_{8}\) & 1.25 & 0.95157896 & 1.00007738 & 0.999960889 & 1 \\
		\(p_{9}\) & 2.5 & 2.08014338 & 2.00018978 & 2.00010483 & 2 \\
		\(p_{10}\) & 1.25 & 0.985076745 & 0.999654308 & 0.999992747 & 1 \\
		\(p_{11}\) & 2.5 & 2.01633511 & 1.9993814 & 1.99988066 & 2 \\
		\(p_{12}\) & 1.25 & 1.259644 & 1.08644736 & 1.00214616 & 1 \\
		\(p_{13}\) & 1.25 & 1.21352542 & 1.0566643 & 1.0001358 & 1 \\
		\(p_{14}\) & 1.25 & 1.00314513 & 0.999433405 & 0.999997189 & 1 \\
		\(p_{15}\) & 2.5 & 2.29280383 & 2.00308053 & 2.00004411 & 2 \\
		\(p_{16}\) & 1.25 & 0.937600975 & 1.00159892 & 1.00001059 & 1 \\
		\(p_{17}\) & 2.5 & 2.10338069 & 1.99518386 & 1.99998034 & 2 \\
		\(p_{18}\) & 1.25 & 1.29358396 & 1.05725502 & 1.00012768 & 1 \\
		\(p_{19}\) & 0.125 & 0.0848720632 & 0.0991639093 & 0.0999808376 & 0.1 \\
		\(p_{20}\) & 1.25 & 1.14647261 & 0.999840949 & 1.00005416 & 1 \\
		\(p_{21}\) & 0.125 & 0.0758080901 & 0.0991754539 & 0.0999778091 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0717687315 & 0.0990283691 & 0.0999856293 & 0.1 \\
		\(p_{23}\) & 1.25 & 1.00612429 & 1.00240141 & 1.00005685 & 1 \\
		\(p_{24}\) & 0.125 & 0.0695497907 & 0.0988764752 & 0.0999821708 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.101169638 & 0.0994929919 & 0.100015632 & 0.1 \\
		\(p_{26}\) & 1.25 & 1.02453053 & 1.00053644 & 0.99991744 & 1 \\
		\(p_{27}\) & 0.125 & 0.101245662 & 0.0994528401 & 0.10002168 & 0.1 \\
		\(p_{28}\) & 1.25 & 1.01680695 & 0.998092821 & 0.999948959 & 1 \\
		\(p_{29}\) & 1.25 & 1.26464586 & 1.01659859 & 1.00039195 & 1 \\
		\(p_{30}\) & 1.25 & 1.34509866 & 0.979133685 & 1.001097 & 1 \\
		\(p_{31}\) & 1.25 & 1.11416822 & 1.00247881 & 1.00009912 & 1 \\
		\(p_{32}\) & 1.25 & 1.24485949 & 1.00895324 & 1.00017191 & 1 \\
		\(p_{33}\) & 1.25 & 1.11535441 & 1.00954907 & 1.00031567 & 1 \\
		\(p_{34}\) & 1.25 & 1.21463232 & 1.00508766 & 1.00022457 & 1 \\
		\(p_{35}\) & 1.25 & 1.31789897 & 1.00739457 & 1.00027132 & 1 \\
		\(p_{36}\) & 1.25 & 0.974290645 & 1.00480178 & 1.00017782 & 1 \\
		$\alpha$ & & 2.95828554 & 0.0116840655 & \num{4.00463919e-07} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points. Regularization parameter \(\alpha\) was determined using \eqref{eq:alphaformula} where \(C = 0.25\) and \(\gamma = 2\).}
\label{tab:tsmn02_21}
\end{table}


==> table/tsmn_21_no_noise_16ds.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{4}$ & $\vecu_{7}$ & $\vecu$ \\ \midrule
			\(p_{1}\) & 1.25 & 1.25512524 & 0.927122051 & 1.00085724 & 1 \\
			\(p_{2}\) & 1.25 & 0.999862712 & 1.00002606 & 1.00000674 & 1 \\
			\(p_{3}\) & 2.5 & 1.97178799 & 1.99991702 & 1.99991175 & 2 \\
			\(p_{4}\) & 1.25 & 0.990143871 & 0.999896404 & 0.999994678 & 1 \\
			\(p_{5}\) & 2.5 & 1.95853912 & 1.99985784 & 1.9999685 & 2 \\
			\(p_{6}\) & 1.25 & 1.25267822 & 0.92718216 & 1.00085391 & 1 \\
			\(p_{7}\) & 1.25 & 1.29546916 & 0.921503261 & 1.00050106 & 1 \\
			\(p_{8}\) & 1.25 & 0.998113434 & 1.0000227 & 1.00001141 & 1 \\
			\(p_{9}\) & 2.5 & 1.9878538 & 2.00007904 & 2.00010144 & 2 \\
			\(p_{10}\) & 1.25 & 1.01372789 & 0.99997927 & 1.00000172 & 1 \\
			\(p_{11}\) & 2.5 & 1.99703695 & 1.99988845 & 1.99997249 & 2 \\
			\(p_{12}\) & 1.25 & 1.29427485 & 0.921414646 & 1.00050365 & 1 \\
			\(p_{13}\) & 1.25 & 1.26093202 & 0.93060889 & 1.00051206 & 1 \\
			\(p_{14}\) & 1.25 & 1.01330944 & 0.999998143 & 1.00006177 & 1 \\
			\(p_{15}\) & 2.5 & 1.94676303 & 1.99988776 & 2.00039646 & 2 \\
			\(p_{16}\) & 1.25 & 0.985547194 & 1.00000026 & 0.999930404 & 1 \\
			\(p_{17}\) & 2.5 & 1.97327136 & 2.00003146 & 2.00004305 & 2 \\
			\(p_{18}\) & 1.25 & 1.27616544 & 0.930140952 & 1.00058938 & 1 \\
			\(p_{19}\) & 0.125 & 0.0843118088 & 0.0997088575 & 0.100006441 & 0.1 \\
			\(p_{20}\) & 1.25 & 0.981821731 & 1.00011001 & 1.00013735 & 1 \\
			\(p_{21}\) & 0.125 & 0.0776212027 & 0.0996417541 & 0.0999985603 & 0.1 \\
			\(p_{22}\) & 0.125 & 0.086556167 & 0.0999725968 & 0.0999951983 & 0.1 \\
			\(p_{23}\) & 1.25 & 0.956213743 & 0.999841926 & 0.99996116 & 1 \\
			\(p_{24}\) & 0.125 & 0.0854886179 & 0.0999785954 & 0.09999813 & 0.1 \\
			\(p_{25}\) & 0.125 & 0.0852485971 & 0.0999880247 & 0.0999983637 & 0.1 \\
			\(p_{26}\) & 1.25 & 0.984253636 & 0.999697311 & 1.00007222 & 1 \\
			\(p_{27}\) & 0.125 & 0.0822077677 & 0.0999874859 & 0.0999931404 & 0.1 \\
			\(p_{28}\) & 1.25 & 0.907849342 & 0.999259411 & 0.999987714 & 1 \\
			\(p_{29}\) & 1.25 & 1.10586514 & 0.999880724 & 0.99978328 & 1 \\
			\(p_{30}\) & 1.25 & 1.34338671 & 1.00104412 & 0.999682621 & 1 \\
			\(p_{31}\) & 1.25 & 1.00716795 & 0.999721591 & 1.0000418 & 1 \\
			\(p_{32}\) & 1.25 & 1.09480976 & 0.999454313 & 0.999775109 & 1 \\
			\(p_{33}\) & 1.25 & 0.986460944 & 0.999899864 & 0.999384976 & 1 \\
			\(p_{34}\) & 1.25 & 0.991171566 & 0.999655209 & 0.999901482 & 1 \\
			\(p_{35}\) & 1.25 & 1.04745953 & 0.99934233 & 0.999822786 & 1 \\
			\(p_{36}\) & 1.25 & 0.974965866 & 1.00029979 & 0.99987451 & 1 \\
			$\alpha$ & & 2.01103137 & 0.00931903131 & \num{2.68809336e-08} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 16 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points. Regularization parameter \(\alpha\) was determined using \eqref{eq:alphaformula} where \(C = 0.005\) and \(\gamma = 2\).}
\label{tab:tsmn01_21}
\end{table}


==> table/tsmn_21_noise_05ds_0p01.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{4}$ & $\vecu_{6}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 1.25 & 1.12356487 & 1.12908183 & 1.12907357 & 1 \\
				\(p_{2}\) & 1.25 & 0.912056317 & 0.893120928 & 0.893122186 & 1 \\
				\(p_{3}\) & 2.5 & 2.361377 & 2.37011999 & 2.37012047 & 2 \\
				\(p_{4}\) & 1.25 & 1.15380988 & 1.1544277 & 1.15442127 & 1 \\
				\(p_{5}\) & 2.5 & 2.48135277 & 2.48582151 & 2.48582064 & 2 \\
				\(p_{6}\) & 1.25 & 1.1337706 & 1.13846794 & 1.13847095 & 1 \\
				\(p_{7}\) & 1.25 & 0.917569394 & 0.91296784 & 0.912964791 & 1 \\
				\(p_{8}\) & 1.25 & 0.853646679 & 0.883403109 & 0.883393186 & 1 \\
				\(p_{9}\) & 2.5 & 2.15099207 & 2.11038105 & 2.11038153 & 2 \\
				\(p_{10}\) & 1.25 & 0.986181058 & 0.991176363 & 0.991186377 & 1 \\
				\(p_{11}\) & 2.5 & 2.10647546 & 2.06396346 & 2.06396698 & 2 \\
				\(p_{12}\) & 1.25 & 0.928244879 & 0.91805048 & 0.918055018 & 1 \\
				\(p_{13}\) & 1.25 & 0.867920028 & 0.856572827 & 0.856566472 & 1 \\
				\(p_{14}\) & 1.25 & 0.95425177 & 0.951146046 & 0.95113649 & 1 \\
				\(p_{15}\) & 2.5 & 2.37981552 & 2.36962985 & 2.36962995 & 2 \\
				\(p_{16}\) & 1.25 & 1.14655982 & 1.13874907 & 1.13875341 & 1 \\
				\(p_{17}\) & 2.5 & 1.84137629 & 1.80137708 & 1.80137968 & 2 \\
				\(p_{18}\) & 1.25 & 0.77134175 & 0.768998253 & 0.769005615 & 1 \\
				\(p_{19}\) & 0.125 & 0.0893828708 & 0.0861897678 & 0.0860159027 & 0.1 \\
				\(p_{20}\) & 1.25 & 1.08297172 & 1.063479 & 1.06348288 & 1 \\
				\(p_{21}\) & 0.125 & 0.084046457 & 0.0830456638 & 0.0830490536 & 0.1 \\
				\(p_{22}\) & 0.125 & 0.0368097853 & 0.0480343796 & 0.0480712995 & 0.1 \\
				\(p_{23}\) & 1.25 & 1.15967762 & 1.12385869 & 1.12386108 & 1 \\
				\(p_{24}\) & 0.125 & 0.0342399104 & 0.0450807034 & 0.0450918511 & 0.1 \\
				\(p_{25}\) & 0.125 & 0.0619096544 & 0.0738841111 & 0.0738324939 & 0.1 \\
				\(p_{26}\) & 1.25 & 1.12306491 & 1.09339195 & 1.09339655 & 1 \\
				\(p_{27}\) & 0.125 & 0.0571527355 & 0.0682349845 & 0.0683073171 & 0.1 \\
				\(p_{28}\) & 1.25 & 0.956115865 & 0.957380949 & 0.95736383 & 1 \\
				\(p_{29}\) & 1.25 & 1.30579922 & 1.31211464 & 1.31210834 & 1 \\
				\(p_{30}\) & 1.25 & 1.31610091 & 1.32584916 & 1.32584775 & 1 \\
				\(p_{31}\) & 1.25 & 1.06706302 & 1.04969832 & 1.04970898 & 1 \\
				\(p_{32}\) & 1.25 & 1.22993218 & 1.23279088 & 1.23278954 & 1 \\
				\(p_{33}\) & 1.25 & 1.000748 & 0.97477555 & 0.974777285 & 1 \\
				\(p_{34}\) & 1.25 & 1.1239445 & 1.09378361 & 1.09378492 & 1 \\
				\(p_{35}\) & 1.25 & 1.37161601 & 1.37816904 & 1.37817114 & 1 \\
				\(p_{36}\) & 1.25 & 0.935572917 & 0.912489292 & 0.9124841 & 1 \\
				$\alpha$ & & 10 & 39.8107171 & \num{1E4} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 1\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points.}
\label{tab:tsmn_21_noise_01}
\end{table}


==> table/tsmn_21_noise_05ds_0p03.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{5}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 1.00597349 & 1.00096765 & 1 \\
		\(p_{2}\) & 1.25 & 0.887295499 & 0.938805859 & 1 \\
		\(p_{3}\) & 2.5 & 2.22631405 & 2.23281743 & 2 \\
		\(p_{4}\) & 1.25 & 1.16973149 & 1.15328019 & 1 \\
		\(p_{5}\) & 2.5 & 2.45009734 & 2.45568659 & 2 \\
		\(p_{6}\) & 1.25 & 1.00228383 & 1.00588121 & 1 \\
		\(p_{7}\) & 1.25 & 0.920876529 & 0.915860361 & 1 \\
		\(p_{8}\) & 1.25 & 0.817403237 & 0.860835142 & 1 \\
		\(p_{9}\) & 2.5 & 2.24315205 & 2.26263733 & 2 \\
		\(p_{10}\) & 1.25 & 1.04816376 & 0.998359302 & 1 \\
		\(p_{11}\) & 2.5 & 2.30771702 & 2.32444832 & 2 \\
		\(p_{12}\) & 1.25 & 0.933039668 & 0.937630717 & 1 \\
		\(p_{13}\) & 1.25 & 0.917997171 & 0.908126007 & 1 \\
		\(p_{14}\) & 1.25 & 0.905250343 & 0.982275776 & 1 \\
		\(p_{15}\) & 2.5 & 2.3901562 & 2.38158796 & 2 \\
		\(p_{16}\) & 1.25 & 1.14838297 & 1.14019231 & 1 \\
		\(p_{17}\) & 2.5 & 1.93301183 & 1.90071228 & 2 \\
		\(p_{18}\) & 1.25 & 0.802913387 & 0.800103483 & 1 \\
		\(p_{19}\) & 0.125 & 0.0747000684 & 0.0870366635 & 0.1 \\
		\(p_{20}\) & 1.25 & 1.14466227 & 1.1218544 & 1 \\
		\(p_{21}\) & 0.125 & 0.0665711446 & 0.0804436992 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0359236546 & 0.034487374 & 0.1 \\
		\(p_{23}\) & 1.25 & 1.36150478 & 1.35522744 & 1 \\
		\(p_{24}\) & 0.125 & 0.0291399644 & 0.0284645732 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.169801914 & 0.189211842 & 0.1 \\
		\(p_{26}\) & 1.25 & 0.933386365 & 0.919063028 & 1 \\
		\(p_{27}\) & 0.125 & 0.183288316 & 0.206006873 & 0.1 \\
		\(p_{28}\) & 1.25 & 1.00891056 & 1.00197555 & 1 \\
		\(p_{29}\) & 1.25 & 1.33356271 & 1.31658897 & 1 \\
		\(p_{30}\) & 1.25 & 1.27713081 & 1.28333144 & 1 \\
		\(p_{31}\) & 1.25 & 1.1543244 & 1.13049412 & 1 \\
		\(p_{32}\) & 1.25 & 1.33091645 & 1.33743077 & 1 \\
		\(p_{33}\) & 1.25 & 1.10916629 & 1.10410547 & 1 \\
		\(p_{34}\) & 1.25 & 1.14649825 & 1.12196986 & 1 \\
		\(p_{35}\) & 1.25 & 1.21865247 & 1.24691715 & 1 \\
		\(p_{36}\) & 1.25 & 1.09510375 & 1.07037661 & 1 \\
		$\alpha$ & & 232.630507 & \num{1E4} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 3\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points.}
\label{tab:tsmn_21_noise_03}
\end{table}


==> table/tsmn_21_noise_05ds_0p05.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{9}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 1.25 & 1.23274011 & 1.23364418 & 1.23364368 & 1 \\
				\(p_{2}\) & 1.25 & 0.960106054 & 0.960484484 & 0.960501931 & 1 \\
				\(p_{3}\) & 2.5 & 2.29121012 & 2.2913277 & 2.29133362 & 2 \\
				\(p_{4}\) & 1.25 & 1.16849544 & 1.16806033 & 1.16802556 & 1 \\
				\(p_{5}\) & 2.5 & 2.54518745 & 2.54556573 & 2.54557343 & 2 \\
				\(p_{6}\) & 1.25 & 1.24253408 & 1.24230741 & 1.2423061 & 1 \\
				\(p_{7}\) & 1.25 & 1.06692056 & 1.06846743 & 1.06849085 & 1 \\
				\(p_{8}\) & 1.25 & 1.04851433 & 1.04939595 & 1.04939188 & 1 \\
				\(p_{9}\) & 2.5 & 2.36005721 & 2.36005694 & 2.36005651 & 2 \\
				\(p_{10}\) & 1.25 & 1.01486897 & 1.01255666 & 1.01254233 & 1 \\
				\(p_{11}\) & 2.5 & 2.22898303 & 2.22856754 & 2.22857211 & 2 \\
				\(p_{12}\) & 1.25 & 1.09028307 & 1.08863744 & 1.08861468 & 1 \\
				\(p_{13}\) & 1.25 & 1.08752816 & 1.08865887 & 1.08866007 & 1 \\
				\(p_{14}\) & 1.25 & 1.02046328 & 1.02178689 & 1.02177452 & 1 \\
				\(p_{15}\) & 2.5 & 2.44898652 & 2.44896428 & 2.44896281 & 2 \\
				\(p_{16}\) & 1.25 & 1.06004769 & 1.05928621 & 1.05930439 & 1 \\
				\(p_{17}\) & 2.5 & 2.20058457 & 2.20055701 & 2.20056939 & 2 \\
				\(p_{18}\) & 1.25 & 0.966109728 & 0.964861575 & 0.964860599 & 1 \\
				\(p_{19}\) & 0.125 & 0.0645199618 & 0.0785915621 & 0.0784355615 & 0.1 \\
				\(p_{20}\) & 1.25 & 1.22288392 & 1.22251664 & 1.22251198 & 1 \\
				\(p_{21}\) & 0.125 & 0.0546697758 & 0.0677831343 & 0.0676376034 & 0.1 \\
				\(p_{22}\) & 0.125 & 0.0589037414 & 0.0570352983 & 0.0570592488 & 0.1 \\
				\(p_{23}\) & 1.25 & 1.18359158 & 1.18338756 & 1.18338887 & 1 \\
				\(p_{24}\) & 0.125 & 0.0529883642 & 0.0515685395 & 0.0515888619 & 0.1 \\
				\(p_{25}\) & 0.125 & 0.0525766655 & 0.0525604351 & 0.0526592918 & 0.1 \\
				\(p_{26}\) & 1.25 & 1.3270365 & 1.32706255 & 1.32707071 & 1 \\
				\(p_{27}\) & 0.125 & 0.0497577452 & 0.0489774445 & 0.0490689529 & 0.1 \\
				\(p_{28}\) & 1.25 & 1.04148835 & 1.04140663 & 1.04136724 & 1 \\
				\(p_{29}\) & 1.25 & 1.45677072 & 1.45720806 & 1.45719468 & 1 \\
				\(p_{30}\) & 1.25 & 1.2160484 & 1.21601745 & 1.21601251 & 1 \\
				\(p_{31}\) & 1.25 & 1.02226594 & 1.02229122 & 1.02229292 & 1 \\
				\(p_{32}\) & 1.25 & 1.20580896 & 1.20558589 & 1.2055894 & 1 \\
				\(p_{33}\) & 1.25 & 1.22659297 & 1.22665897 & 1.22665797 & 1 \\
				\(p_{34}\) & 1.25 & 1.29687298 & 1.29705577 & 1.29707419 & 1 \\
				\(p_{35}\) & 1.25 & 1.36690693 & 1.36681746 & 1.36682422 & 1 \\
				\(p_{36}\) & 1.25 & 1.28030652 & 1.28061177 & 1.28060074 & 1 \\
				$\alpha$ & & 92.6118728 & \num{1E4} & \num{1E4} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 5\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), i.e. 20 time points.}
\label{tab:tsmn_21_noise_05}
\end{table}


==> table/tsmn_no_noise_05ds.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSS SSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{10}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 1.23403125 & 1.04970674 & 1.00020433 & 1 \\
		\(p_{2}\) & 1.25 & 0.979737257 & 0.999533015 & 1.00022216 & 1 \\
		\(p_{3}\) & 2.5 & 2.02379893 & 2.00154505 & 1.99951318 & 2 \\
		\(p_{4}\) & 1.25 & 0.912416376 & 0.999165534 & 0.999986751 & 1 \\
		\(p_{5}\) & 2.5 & 1.66310201 & 1.99780302 & 1.99999288 & 2 \\
		\(p_{6}\) & 1.25 & 1.23230973 & 1.04979776 & 1.0002031 & 1 \\
		\(p_{7}\) & 1.25 & 1.2468322 & 1.08048517 & 1.0004875 & 1 \\
		\(p_{8}\) & 1.25 & 0.980261882 & 1.00201878 & 0.999968907 & 1 \\
		\(p_{9}\) & 2.5 & 2.01511216 & 1.99619245 & 2.00009361 & 2 \\
		\(p_{10}\) & 1.25 & 0.999491406 & 0.999705992 & 0.999999413 & 1 \\
		\(p_{11}\) & 2.5 & 1.9835515 & 2.00172762 & 1.9998918 & 2 \\
		\(p_{12}\) & 1.25 & 1.24622666 & 1.08086691 & 1.00047922 & 1 \\
		\(p_{13}\) & 1.25 & 1.2373248 & 1.19626312 & 1.00171945 & 1 \\
		\(p_{14}\) & 1.25 & 0.986985299 & 0.997799053 & 1.00005545 & 1 \\
		\(p_{15}\) & 2.5 & 2.01116699 & 2.00851643 & 1.99988298 & 2 \\
		\(p_{16}\) & 1.25 & 0.982419647 & 1.00648045 & 0.999872548 & 1 \\
		\(p_{17}\) & 2.5 & 2.01684864 & 1.98551115 & 2.00019573 & 2 \\
		\(p_{18}\) & 1.25 & 1.25695336 & 1.18965251 & 1.00184079 & 1 \\
		\(p_{19}\) & 0.125 & 0.0917582168 & 0.0986762348 & 0.0999975188 & 0.1 \\
		\(p_{20}\) & 1.25 & 1.00798604 & 0.999589428 & 1.00006192 & 1 \\
		\(p_{21}\) & 0.125 & 0.0903847433 & 0.0986888608 & 0.0999940189 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0913840058 & 0.0991582262 & 0.100001411 & 0.1 \\
		\(p_{23}\) & 1.25 & 0.983998278 & 1.00381168 & 1.0000288 & 1 \\
		\(p_{24}\) & 0.125 & 0.092231548 & 0.0989238031 & 0.0999997043 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.101216535 & 0.0989387414 & 0.0999975974 & 0.1 \\
		\(p_{26}\) & 1.25 & 1.01751255 & 1.00223215 & 0.999960958 & 1 \\
		\(p_{27}\) & 0.125 & 0.100319739 & 0.0987919747 & 0.100000705 & 0.1 \\
		\(p_{28}\) & 1.25 & 0.991738151 & 0.997033015 & 0.999993611 & 1 \\
		\(p_{29}\) & 1.25 & 1.1773919 & 1.03158457 & 1.00010507 & 1 \\
		\(p_{30}\) & 1.25 & 1.38590407 & 1.06046653 & 1.00025053 & 1 \\
		\(p_{31}\) & 1.25 & 1.05282649 & 1.00624042 & 1.00003599 & 1 \\
		\(p_{32}\) & 1.25 & 1.15774435 & 1.02030939 & 1.00000591 & 1 \\
		\(p_{33}\) & 1.25 & 1.15440728 & 1.03604956 & 0.999941151 & 1 \\
		\(p_{34}\) & 1.25 & 1.09691258 & 1.01650049 & 1.00006984 & 1 \\
		\(p_{35}\) & 1.25 & 1.15120239 & 1.02209026 & 1.00010126 & 1 \\
		\(p_{36}\) & 1.25 & 1.01470895 & 1.01037296 & 1.00008351 & 1 \\
		$\alpha$ & & 0.334783777 & 0.0396352653 & \num{2.51783961E-4} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was determined using \eqref{eq:alphaformula} where \(C = 0.25\) and \(\gamma = 1\).}
\label{tab:tsmn02}
\end{table}


==> table/tsmn_no_noise_05ds_21.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSS SSS}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{10}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 1.2468801 & 0.999211744 & 1.00116246 & 1 \\
		\(p_{2}\) & 1.25 & 0.929354096 & 0.999788621 & 1.00020968 & 1 \\
		\(p_{3}\) & 2.5 & 2.28327634 & 2.0006259 & 1.999535 & 2 \\
		\(p_{4}\) & 1.25 & 1.17855316 & 0.999606704 & 0.999982026 & 1 \\
		\(p_{5}\) & 2.5 & 2.54455663 & 1.998669 & 1.99998259 & 2 \\
		\(p_{6}\) & 1.25 & 1.2562049 & 0.999315372 & 1.00116117 & 1 \\
		\(p_{7}\) & 1.25 & 1.24491525 & 1.08624586 & 1.00215195 & 1 \\
		\(p_{8}\) & 1.25 & 0.95157896 & 1.00007738 & 0.999960889 & 1 \\
		\(p_{9}\) & 2.5 & 2.08014338 & 2.00018978 & 2.00010483 & 2 \\
		\(p_{10}\) & 1.25 & 0.985076745 & 0.999654308 & 0.999992747 & 1 \\
		\(p_{11}\) & 2.5 & 2.01633511 & 1.9993814 & 1.99988066 & 2 \\
		\(p_{12}\) & 1.25 & 1.259644 & 1.08644736 & 1.00214616 & 1 \\
		\(p_{13}\) & 1.25 & 1.21352542 & 1.0566643 & 1.0001358 & 1 \\
		\(p_{14}\) & 1.25 & 1.00314513 & 0.999433405 & 0.999997189 & 1 \\
		\(p_{15}\) & 2.5 & 2.29280383 & 2.00308053 & 2.00004411 & 2 \\
		\(p_{16}\) & 1.25 & 0.937600975 & 1.00159892 & 1.00001059 & 1 \\
		\(p_{17}\) & 2.5 & 2.10338069 & 1.99518386 & 1.99998034 & 2 \\
		\(p_{18}\) & 1.25 & 1.29358396 & 1.05725502 & 1.00012768 & 1 \\
		\(p_{19}\) & 0.125 & 0.0848720632 & 0.0991639093 & 0.0999808376 & 0.1 \\
		\(p_{20}\) & 1.25 & 1.14647261 & 0.999840949 & 1.00005416 & 1 \\
		\(p_{21}\) & 0.125 & 0.0758080901 & 0.0991754539 & 0.0999778091 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0717687315 & 0.0990283691 & 0.0999856293 & 0.1 \\
		\(p_{23}\) & 1.25 & 1.00612429 & 1.00240141 & 1.00005685 & 1 \\
		\(p_{24}\) & 0.125 & 0.0695497907 & 0.0988764752 & 0.0999821708 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.101169638 & 0.0994929919 & 0.100015632 & 0.1 \\
		\(p_{26}\) & 1.25 & 1.02453053 & 1.00053644 & 0.99991744 & 1 \\
		\(p_{27}\) & 0.125 & 0.101245662 & 0.0994528401 & 0.10002168 & 0.1 \\
		\(p_{28}\) & 1.25 & 1.01680695 & 0.998092821 & 0.999948959 & 1 \\
		\(p_{29}\) & 1.25 & 1.26464586 & 1.01659859 & 1.00039195 & 1 \\
		\(p_{30}\) & 1.25 & 1.34509866 & 0.979133685 & 1.001097 & 1 \\
		\(p_{31}\) & 1.25 & 1.11416822 & 1.00247881 & 1.00009912 & 1 \\
		\(p_{32}\) & 1.25 & 1.24485949 & 1.00895324 & 1.00017191 & 1 \\
		\(p_{33}\) & 1.25 & 1.11535441 & 1.00954907 & 1.00031567 & 1 \\
		\(p_{34}\) & 1.25 & 1.21463232 & 1.00508766 & 1.00022457 & 1 \\
		\(p_{35}\) & 1.25 & 1.31789897 & 1.00739457 & 1.00027132 & 1 \\
		\(p_{36}\) & 1.25 & 0.974290645 & 1.00480178 & 1.00017782 & 1 \\
		$\alpha$ & & 2.95828554 & 0.0116840655 & \num{4.00463919e-07} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{With 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), which gives us 20 time points. We found \(\alpha\) as a function of the residual where \(C = 0.25\) and \(S = 2\). }
\label{tab:tsmn02_21}
\end{table}


==> table/tsmn_no_noise_05ds_initial_10p0.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSS}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{4}$ & $\vecu_{8}$ & $\vecu_{13}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 11 & 1.87380445 & 1.22553735 & 1.00003798 & 1 \\
		\(p_{2}\) & 11 & 1.85882173 & 0.710211101 & 0.999999676 & 1 \\
		\(p_{3}\) & 22 & 3.71902864 & 2.22716427 & 2.00000072 & 2 \\
		\(p_{4}\) & 11 & 1.79624649 & 1.13154998 & 1.00000016 & 1 \\
		\(p_{5}\) & 22 & 3.71367072 & 2.27565112 & 2.00000028 & 2 \\
		\(p_{6}\) & 11 & 1.89565039 & 1.23407447 & 1.00003798 & 1 \\
		\(p_{7}\) & 11 & 1.86227315 & 1.26251334 & 1.00001399 & 1 \\
		\(p_{8}\) & 11 & 1.85953931 & 0.733905632 & 0.999999867 & 1 \\
		\(p_{9}\) & 22 & 3.71874747 & 2.33940612 & 2.0000005 & 2 \\
		\(p_{10}\) & 11 & 1.81931617 & 1.03153321 & 0.999999957 & 1 \\
		\(p_{11}\) & 22 & 3.70445422 & 2.14272669 & 1.9999996 & 2 \\
		\(p_{12}\) & 11 & 1.89676548 & 1.28255148 & 1.00001397 & 1 \\
		\(p_{13}\) & 11 & 1.86520005 & 1.20648773 & 1.00000539 & 1 \\
		\(p_{14}\) & 11 & 1.85936855 & 0.906817234 & 1.00000163 & 1 \\
		\(p_{15}\) & 22 & 3.71878322 & 2.48130735 & 1.9999936 & 2 \\
		\(p_{16}\) & 11 & 1.83164854 & 0.906483098 & 0.999995049 & 1 \\
		\(p_{17}\) & 22 & 3.71005836 & 2.25031044 & 2.0000083 & 2 \\
		\(p_{18}\) & 11 & 1.87528594 & 1.36867812 & 1.00000987 & 1 \\
		\(p_{19}\) & 1.1 & 0.188313118 & 0.0777837256 & 0.099999585 & 0.1 \\
		\(p_{20}\) & 11 & 1.85866625 & 1.20626852 & 0.999998971 & 1 \\
		\(p_{21}\) & 1.1 & 0.2084057 & 0.0699187791 & 0.09999964 & 0.1 \\
		\(p_{22}\) & 1.1 & 0.180413866 & 0.0637095893 & 0.0999998279 & 0.1 \\
		\(p_{23}\) & 11 & 1.85665484 & 1.11758015 & 1.00000029 & 1 \\
		\(p_{24}\) & 1.1 & 0.179736285 & 0.0584440909 & 0.0999998101 & 0.1 \\
		\(p_{25}\) & 1.1 & 0.264423093 & 0.104072391 & 0.0999997149 & 0.1 \\
		\(p_{26}\) & 11 & 1.84760546 & 1.20857812 & 1.0000006 & 1 \\
		\(p_{27}\) & 1.1 & 0.0773214794 & 0.0914279974 & 0.0999996725 & 0.1 \\
		\(p_{28}\) & 11 & 1.84745717 & 1.00365891 & 0.999999737 & 1 \\
		\(p_{29}\) & 11 & 1.86385436 & 1.3943034 & 0.999995915 & 1 \\
		\(p_{30}\) & 11 & 1.85679386 & 1.34526678 & 0.999997941 & 1 \\
		\(p_{31}\) & 11 & 1.85344637 & 1.07078838 & 0.999998849 & 1 \\
		\(p_{32}\) & 11 & 1.86292966 & 1.40400697 & 0.999996316 & 1 \\
		\(p_{33}\) & 11 & 1.85762688 & 1.22465943 & 1.00000091 & 1 \\
		\(p_{34}\) & 11 & 1.87273882 & 1.17688023 & 0.999998651 & 1 \\
		\(p_{35}\) & 11 & 1.85184421 & 1.47447858 & 0.999996131 & 1 \\
		\(p_{36}\) & 11 & 1.8595039 & 1.02236049 & 1.00000176 & 1 \\
		$\alpha$ & & 212.749466 & 0.0567469565 & 3.41739628e-12 &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{With 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), which gives us 241 data points. For our guess we use . We found \(\alpha\) as a function of the residual. }
\label{tab:tsmn_far}
\end{table}


==> table/tsmn_no_noise_05ds_initial_1p5.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSS}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{14}$ & $\vecu_{28}$ & $\vecu_{53}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 2 & 1.87958234 & 2.00340254 & 0.999907509 & 1 \\
		\(p_{2}\) & 2 & 1.98044868 & 0.843874705 & 0.999984674 & 1 \\
		\(p_{3}\) & 4 & 3.98364986 & 2.89112008 & 2.00003083 & 2 \\
		\(p_{4}\) & 2 & 1.18593687 & 1.45621917 & 1.00000333 & 1 \\
		\(p_{5}\) & 4 & 4.07703314 & 4.0312742 & 2.00000318 & 2 \\
		\(p_{6}\) & 2 & 2.11640663 & 2.04293005 & 0.999907167 & 1 \\
		\(p_{7}\) & 2 & 1.77869821 & 2.017065 & 1.00009072 & 1 \\
		\(p_{8}\) & 2 & 1.95899365 & 1.23899561 & 1.00002247 & 1 \\
		\(p_{9}\) & 4 & 3.98044092 & 1.3418938 & 1.99994597 & 2 \\
		\(p_{10}\) & 2 & 0.936659576 & 1.01457866 & 1.00000092 & 1 \\
		\(p_{11}\) & 4 & 3.89418984 & 2.38843051 & 2.00004648 & 2 \\
		\(p_{12}\) & 2 & 2.20911299 & 2.03726633 & 1.00009459 & 1 \\
		\(p_{13}\) & 2 & 2.23539707 & 2.21945298 & 1.00026127 & 1 \\
		\(p_{14}\) & 2 & 1.97950408 & 0.964051337 & 0.999913069 & 1 \\
		\(p_{15}\) & 4 & 3.99286012 & 3.5182503 & 2.0002788 & 2 \\
		\(p_{16}\) & 2 & 1.28868905 & 1.22313344 & 1.00024269 & 1 \\
		\(p_{17}\) & 4 & 3.67072254 & 1.63523123 & 1.99957483 & 2 \\
		\(p_{18}\) & 2 & 1.75094596 & 1.89470673 & 1.00004095 & 1 \\
		\(p_{19}\) & 0.2 & 0.10405191 & 0.0906324398 & 0.0999994114 & 0.1 \\
		\(p_{20}\) & 2 & 1.92580072 & 1.66858886 & 0.999970547 & 1 \\
		\(p_{21}\) & 0.2 & 0.0692520954 & 0.0653892739 & 0.100000989 & 0.1 \\
		\(p_{22}\) & 0.2 & 0.0664801093 & 0.0569105558 & 0.0999973866 & 0.1 \\
		\(p_{23}\) & 2 & 1.85729629 & 0.808388193 & 1.00000306 & 1 \\
		\(p_{24}\) & 0.2 & 0.0385187236 & 0.0623106783 & 0.0999971608 & 0.1 \\
		\(p_{25}\) & 0.2 & 0.0150365919 & 0.044541491 & 0.100005151 & 0.1 \\
		\(p_{26}\) & 2 & 2.20397962 & 1.64869965 & 1.00000425 & 1 \\
		\(p_{27}\) & 0.2 & 0.0108934463 & 0.0314197628 & 0.100004853 & 0.1 \\
		\(p_{28}\) & 2 & 1.31271933 & 1.07768214 & 0.999997408 & 1 \\
		\(p_{29}\) & 2 & 1.60082758 & 1.74123237 & 0.999983219 & 1 \\
		\(p_{30}\) & 2 & 1.88962347 & 1.17353226 & 0.999956733 & 1 \\
		\(p_{31}\) & 2 & 1.4365254 & 1.11806022 & 0.999973607 & 1 \\
		\(p_{32}\) & 2 & 2.11409405 & 2.11824589 & 0.999987335 & 1 \\
		\(p_{33}\) & 2 & 1.95554621 & 2.01649063 & 1.00005527 & 1 \\
		\(p_{34}\) & 2 & 2.60839522 & 2.03599787 & 0.999966337 & 1 \\
		\(p_{35}\) & 2 & 2.15880185 & 3.39525688 & 0.999950094 & 1 \\
		\(p_{36}\) & 2 & 1.24630048 & 1.07603429 & 0.999981409 & 1 \\
		$\alpha$ & & 30.9175967 & 9.93356485 & 1.53429779e-05 &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{ With 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), which gives us 241 data points. We found \(\alpha\) as a function of the residual. }
\label{tab:tsmn03}
\end{table}


==> table/tsmn_no_noise_05ds_type1_lower.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{3}$ & $\vecu_{6}$ & $\vecu_{9}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 0.5 & 0.626169343 & 0.977716285 & 0.999466903 & 1 \\
				\(p_{2}\) & 0.5 & 0.845634234 & 1.00165165 & 1.00032001 & 1 \\
				\(p_{3}\) & 1 & 2.0765202 & 1.99579683 & 1.99928762 & 2 \\
				\(p_{4}\) & 0.5 & 0.982500076 & 0.999143968 & 1.00000904 & 1 \\
				\(p_{5}\) & 1 & 1.93297677 & 1.9974715 & 2.00007038 & 2 \\
				\(p_{6}\) & 0.5 & 0.626182785 & 0.977572525 & 0.999464198 & 1 \\
				\(p_{7}\) & 0.5 & 0.671518537 & 0.953503371 & 0.999077883 & 1 \\
				\(p_{8}\) & 0.5 & 1.03057903 & 1.00300404 & 0.999621733 & 1 \\
				\(p_{9}\) & 1 & 1.92455521 & 1.99137497 & 2.00094515 & 2 \\
				\(p_{10}\) & 0.5 & 1.01632026 & 0.999800663 & 0.999996089 & 1 \\
				\(p_{11}\) & 1 & 1.84023294 & 2.00283954 & 1.99917418 & 2 \\
				\(p_{12}\) & 0.5 & 0.670292065 & 0.952887657 & 0.999007177 & 1 \\
				\(p_{13}\) & 0.5 & 0.516679575 & 0.707435771 & 1.00020266 & 1 \\
				\(p_{14}\) & 0.5 & 0.473021861 & 1.00527371 & 0.999925276 & 1 \\
				\(p_{15}\) & 1 & 1.96004889 & 1.88135825 & 2.00036001 & 2 \\
				\(p_{16}\) & 0.5 & 0.700850149 & 0.999722595 & 1.00025748 & 1 \\
				\(p_{17}\) & 1 & 2.05684542 & 1.99358403 & 1.99949396 & 2 \\
				\(p_{18}\) & 0.5 & 0.568752803 & 0.71415055 & 1.00001564 & 1 \\
				\(p_{19}\) & 0.05 & 0.0897168063 & 0.10109981 & 0.100016518 & 0.1 \\
				\(p_{20}\) & 0.5 & 0.833640832 & 1.00321024 & 1.00004308 & 1 \\
				\(p_{21}\) & 0.05 & 0.0995106361 & 0.100882453 & 0.100007884 & 0.1 \\
				\(p_{22}\) & 0.05 & 0.108314217 & 0.0966272839 & 0.100041958 & 0.1 \\
				\(p_{23}\) & 0.5 & 0.9367499 & 0.992308113 & 1.00000115 & 1 \\
				\(p_{24}\) & 0.05 & 0.109959988 & 0.0973377171 & 0.100045607 & 0.1 \\
				\(p_{25}\) & 0.05 & 0.115357994 & 0.0985938387 & 0.09997673 & 0.1 \\
				\(p_{26}\) & 0.5 & 0.960168927 & 1.00582109 & 0.999940974 & 1 \\
				\(p_{27}\) & 0.05 & 0.119977894 & 0.0984232961 & 0.0999833641 & 0.1 \\
				\(p_{28}\) & 0.5 & 0.936869863 & 1.00424307 & 1.00004586 & 1 \\
				\(p_{29}\) & 0.5 & 1.07953988 & 0.937323965 & 0.999448726 & 1 \\
				\(p_{30}\) & 0.5 & 1.03893284 & 0.819932069 & 0.998213778 & 1 \\
				\(p_{31}\) & 0.5 & 0.884891983 & 0.983656439 & 0.999804116 & 1 \\
				\(p_{32}\) & 0.5 & 1.16724837 & 0.955376413 & 0.999530553 & 1 \\
				\(p_{33}\) & 0.5 & 1.34060165 & 0.919583822 & 0.999417408 & 1 \\
				\(p_{34}\) & 0.5 & 0.969341925 & 0.960231357 & 0.999696185 & 1 \\
				\(p_{35}\) & 0.5 & 1.11884215 & 0.94311075 & 0.99961493 & 1 \\
				\(p_{36}\) & 0.5 & 1.00013253 & 0.97423824 & 0.999934331 & 1 \\
				$\alpha$ & & 1.1659144 & 0.0158489319 & \num{10000} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{ The evolution of the parameters at select iterations, with 5 data sets, \((\mathbf{u}_{0} = 0.5\mathbf{u}\), \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was chosen optimally.}
\label{tab:tsmn_type1_lower}
\end{table}


==> table/tsmn_no_noise_05ds_type1_upper.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{4}$ & $\vecu_{8}$ & $\vecu_{13}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.65 & 1.65154512 & 1.10582061 & 0.999941119 & 1 \\
		\(p_{2}\) & 1.65 & 0.911543937 & 1.00060448 & 1.00023796 & 1 \\
		\(p_{3}\) & 3.3 & 2.11606522 & 1.98043451 & 1.99947636 & 2 \\
		\(p_{4}\) & 1.65 & 1.37818007 & 0.996263774 & 0.999997825 & 1 \\
		\(p_{5}\) & 3.3 & 3.34476125 & 1.98821385 & 2.00002616 & 2 \\
		\(p_{6}\) & 1.65 & 1.66243694 & 1.10768263 & 0.999939695 & 1 \\
		\(p_{7}\) & 1.65 & 1.62798194 & 1.04003786 & 1.00010144 & 1 \\
		\(p_{8}\) & 1.65 & 0.589713379 & 1.00723876 & 0.999865972 & 1 \\
		\(p_{9}\) & 3.3 & 2.59395611 & 1.98375468 & 2.00034833 & 2 \\
		\(p_{10}\) & 1.65 & 1.00120368 & 0.999993491 & 0.999997985 & 1 \\
		\(p_{11}\) & 3.3 & 2.19627718 & 2.0097998 & 1.99967536 & 2 \\
		\(p_{12}\) & 1.65 & 1.68033621 & 1.04308703 & 1.00007423 & 1 \\
		\(p_{13}\) & 1.65 & 1.60892755 & 1.02538096 & 1.00421863 & 1 \\
		\(p_{14}\) & 1.65 & 0.711963147 & 1.04766376 & 0.999943043 & 1 \\
		\(p_{15}\) & 3.3 & 2.90314574 & 2.00676187 & 2.00028435 & 2 \\
		\(p_{16}\) & 1.65 & 0.894844361 & 0.690988968 & 1.00021213 & 1 \\
		\(p_{17}\) & 3.3 & 1.59231429 & 1.97613075 & 1.99957703 & 2 \\
		\(p_{18}\) & 1.65 & 1.75823026 & 1.33471615 & 1.00402852 & 1 \\
		\(p_{19}\) & 0.165 & 0.0763454566 & 0.0962454009 & 0.100004483 & 0.1 \\
		\(p_{20}\) & 1.65 & 1.33163519 & 1.00149646 & 1.00005653 & 1 \\
		\(p_{21}\) & 0.165 & 0.0616561195 & 0.0962847916 & 0.100001233 & 0.1 \\
		\(p_{22}\) & 0.165 & 0.036062972 & 0.0966315734 & 0.100012542 & 0.1 \\
		\(p_{23}\) & 1.65 & 0.805532313 & 1.00313698 & 1.00001893 & 1 \\
		\(p_{24}\) & 0.165 & 0.048024189 & 0.0964791112 & 0.100011591 & 0.1 \\
		\(p_{25}\) & 0.165 & 0.149164203 & 0.0972871611 & 0.0999831882 & 0.1 \\
		\(p_{26}\) & 1.65 & 1.85689152 & 0.990514266 & 0.999995336 & 1 \\
		\(p_{27}\) & 0.165 & 0.0889069795 & 0.0972255875 & 0.099983913 & 0.1 \\
		\(p_{28}\) & 1.65 & 0.993898935 & 0.989120809 & 1.00002612 & 1 \\
		\(p_{29}\) & 1.65 & 1.67235354 & 1.07317889 & 0.999770286 & 1 \\
		\(p_{30}\) & 1.65 & 1.76172836 & 0.681673771 & 0.999427954 & 1 \\
		\(p_{31}\) & 1.65 & 1.26886457 & 1.01622208 & 0.99994131 & 1 \\
		\(p_{32}\) & 1.65 & 1.64414958 & 1.03644581 & 0.99978963 & 1 \\
		\(p_{33}\) & 1.65 & 0.790454336 & 1.05041051 & 0.999667741 & 1 \\
		\(p_{34}\) & 1.65 & 1.59914879 & 1.02303316 & 0.999886605 & 1 \\
		\(p_{35}\) & 1.65 & 2.15907508 & 1.01667977 & 0.999849086 & 1 \\
		\(p_{36}\) & 1.65 & 1.34886262 & 1.02773832 & 0.999978879 & 1 \\
		$\alpha$ & & 2.51188643 & 0.0158489319 & \num{10000} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{ The evolution of the parameters at select iterations, with 5 data sets, \((\mathbf{u}_{0} = 1.65\mathbf{u}\), \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was chosen near optimally.}
\label{tab:tsmn_type1_upper}
\end{table}


==> table/tsmn_no_noise_05ds_type2_large.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lcSSc}
		\toprule
		$\vecu$ &		$\vecu_{0}$ &$\vecu_{4}$ &		$\vecu_{7}$ &		$\vecu$ \\ \midrule
		\(p_{1}\) &		1001 &			0.999208266 &		0.999984856 &		1 \\
		\(p_{2}\) &		1001 &			0.90059317 &		0.999814185 &		1 \\
		\(p_{3}\) &		2002 &			1.92904842 &		2.00044144 &		2 \\
		\(p_{4}\) &		1001 &			0.985491774 &		1.00000773 &		1 \\
		\(p_{5}\) &		2002 &			1.96085245 &		1.99998514 &		2 \\
		\(p_{6}\) &		1001 &			1.0002895 &		0.999987515 &		1 \\
		\(p_{7}\) &		1001 &			0.764392822 &		0.999994458 &		1 \\
		\(p_{8}\) &		1001 &			0.989047087 &		0.999998442 &		1 \\
		\(p_{9}\) &		2002 &			2.02527479 &		2.00002122 &		2 \\
		\(p_{10}\) &		1001 &		0.997282544 &		1.00000262 &		1 \\
		\(p_{11}\) &		2002 &		1.97481006 &		1.99998739 &		2 \\
		\(p_{12}\) &		1001 &		0.775715024 &		0.999992853 &		1 \\
		\(p_{13}\) &		1001 &		1.36471944 &		1.00044208 &		1 \\
		\(p_{14}\) &		1001 &		0.970241059 &		0.999993283 &		1 \\
		\(p_{15}\) &		2002 &		1.78164566 &		2.00012783 &		2 \\
		\(p_{16}\) &		1001 &		1.10567168 &		0.999983438 &		1 \\
		\(p_{17}\) &		2002 &		1.8461203 &		1.99988786 &		2 \\
		\(p_{18}\) &		1001 &		1.20949489 &		1.00045223 &		1 \\
		\(p_{19}\) &		100.1 &		0.0993028393 &		0.0999996696 &		0.1 \\
		\(p_{20}\) &		1001 &		0.94542369 &		1.00002265 &		1 \\
		\(p_{21}\) &		100.1 &			0.0960059355 &		0.0999984126 &		0.1 \\
		\(p_{22}\) &		100.1 &			0.0865541638 &		0.100004127 &		0.1 \\
		\(p_{23}\) &		1001 &		0.950801306 &		1.00000427 &		1 \\
		\(p_{24}\) &		100.1 &			0.0893215641 &		0.100003889 &		0.1 \\
		\(p_{25}\) &		100.1 &			0.0868776771 &		0.100010301 &		0.1 \\
		\(p_{26}\) &		1001 &		0.931344031 &		0.999950161 &		1 \\
		\(p_{27}\) &		100.1 &			0.0906729597 &		0.100013913 &		0.1 \\
		\(p_{28}\) &		1001 &		0.994721876 &		0.999989592 &		1 \\
		\(p_{29}\) &		1001 &		1.03187899 &		1.00003769 &		1 \\
		\(p_{30}\) &		1001 &		0.962557002 &		1.00008717 &		1 \\
		\(p_{31}\) &		1001 &		1.01904878 &		0.999969937 &		1 \\
		\(p_{32}\) &		1001 &		0.955442453 &		1.00001186 &		1 \\
		\(p_{33}\) &		1001 &		0.929475332 &		1.00014221 &		1 \\
		\(p_{34}\) &		1001 &		0.920077767 &		0.999981887 &		1 \\
		\(p_{35}\) &		1001 &		0.762934985 &		0.999974769 &		1 \\
		\(p_{36}\) &		1001 &		1.01245573 &		1.0000074 &		1 \\
		$\alpha$ &		&					\num{7.94328235e-06} &		1e-06 &		 \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{ The evolution of the parameters at select iterations, with 5 data sets, type 2 regularization, \((\mathbf{u}_{0} = 1001\mathbf{u}\), \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was chosen near optimally.}
\label{tab:tsmn_type2_large}
\end{table}


==> table/tsmn_no_noise_05ds_type2_small.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{4}$ & $\vecu_{8}$ & $\vecu_{14}$ & $\vecu$ \\ \midrule
\(p_{1}\) & 0.03 & 0.737221345 & 0.963897509 & 0.9999746 & 1 \\
\(p_{2}\) & 0.03 & 1.15114232 & 1.20072628 & 1.00024257 & 1 \\
\(p_{3}\) & 0.06 & 1.52136211 & 1.60084001 & 1.99945885 & 2 \\
\(p_{4}\) & 0.03 & 0.875455828 & 0.959864577 & 0.999992984 & 1 \\
\(p_{5}\) & 0.06 & 1.71421694 & 1.92922185 & 2.00001648 & 2 \\
\(p_{6}\) & 0.03 & 0.721197625 & 0.960669483 & 0.999973092 & 1 \\
\(p_{7}\) & 0.03 & 0.618656745 & 0.87370521 & 0.999926014 & 1 \\
\(p_{8}\) & 0.03 & 0.772749076 & 1.03786452 & 0.999994507 & 1 \\
\(p_{9}\) & 0.06 & 2.00588681 & 1.74846142 & 2.00001558 & 2 \\
\(p_{10}\) & 0.03 & 0.927440217 & 0.994637987 & 1.00000179 & 1 \\
\(p_{11}\) & 0.06 & 1.36225492 & 2.00313025 & 1.99997863 & 2 \\
\(p_{12}\) & 0.03 & 0.55949302 & 0.857172219 & 0.999923418 & 1 \\
\(p_{13}\) & 0.03 & 0.536878353 & 0.942787928 & 1.00019823 & 1 \\
\(p_{14}\) & 0.03 & 0.48765519 & 1.14685544 & 0.999985423 & 1 \\
\(p_{15}\) & 0.06 & 1.53861529 & 1.30604422 & 2.00007362 & 2 \\
\(p_{16}\) & 0.03 & 1.09438682 & 0.963918741 & 1.00005075 & 1 \\
\(p_{17}\) & 0.06 & 1.72292748 & 2.03810911 & 1.99991809 & 2 \\
\(p_{18}\) & 0.03 & 0.462456281 & 1.07505591 & 1.00015257 & 1 \\
\(p_{19}\) & 0.003 & 0.0838553321 & 0.0890382732 & 0.100002039 & 0.1 \\
\(p_{20}\) & 0.03 & 0.982137681 & 0.836518754 & 1.0000039 & 1 \\
\(p_{21}\) & 0.003 & 0.0803601411 & 0.0962289846 & 0.1000018 & 0.1 \\
\(p_{22}\) & 0.003 & 0.140838617 & 0.0516910857 & 0.100004647 & 0.1 \\
\(p_{23}\) & 0.03 & 0.806694359 & 0.622618555 & 1.00000089 & 1 \\
\(p_{24}\) & 0.003 & 0.156229259 & 0.0654196304 & 0.100004619 & 0.1 \\
\(p_{25}\) & 0.003 & 0.141181087 & 0.0306196026 & 0.100011754 & 0.1 \\
\(p_{26}\) & 0.03 & 0.654611369 & 0.184156298 & 0.999958615 & 1 \\
\(p_{27}\) & 0.003 & 0.177855041 & 0.0476447887 & 0.100014776 & 0.1 \\
\(p_{28}\) & 0.03 & 0.521965528 & 0.936343126 & 1.00000017 & 1 \\
\(p_{29}\) & 0.03 & 0.813259557 & 0.545624573 & 0.99989085 & 1 \\
\(p_{30}\) & 0.03 & 0.267789203 & 0.658218793 & 0.99976338 & 1 \\
\(p_{31}\) & 0.03 & 0.420731593 & 0.889447347 & 0.9999534 & 1 \\
\(p_{32}\) & 0.03 & -0.207561844 & 0.796603238 & 0.999869422 & 1 \\
\(p_{33}\) & 0.03 & 0.654626818 & 0.733923164 & 0.999843052 & 1 \\
\(p_{34}\) & 0.03 & 0.475655459 & 1.04739015 & 0.999897904 & 1 \\
\(p_{35}\) & 0.03 & 0.0644793881 & 1.20461925 & 0.999845741 & 1 \\
\(p_{36}\) & 0.03 & 0.894142978 & 1.13424669 & 0.999963266 & 1 \\
$\alpha$ & & 0.1 & 0.0125892541 & 1e-06 &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{ The evolution of the parameters at select iterations, with 5 data sets, type 2 regularization, \((\mathbf{u}_{0} = 0.03 \mathbf{u}\), \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was chosen near optimally.}
\label{tab:tsmn_type2_small}
\end{table}


==> table/tsmn_no_noise_16ds.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{4}$ & $\vecu_{7}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 1.25 & 1.24638544 & 0.952769935 & 1.00114463 & 1 \\
				\(p_{2}\) & 1.25 & 1.00144721 & 1.00011747 & 1.00001193 & 1 \\
				\(p_{3}\) & 2.5 & 2.01250641 & 2.00011472 & 1.9999059 & 2 \\
				\(p_{4}\) & 1.25 & 0.987740455 & 1.00011948 & 0.999989635 & 1 \\
				\(p_{5}\) & 2.5 & 2.00416156 & 1.99971343 & 1.99996135 & 2 \\
				\(p_{6}\) & 1.25 & 1.25030262 & 0.952721554 & 1.00114352 & 1 \\
				\(p_{7}\) & 1.25 & 1.28520602 & 0.969968 & 1.00059758 & 1 \\
				\(p_{8}\) & 1.25 & 0.991183426 & 1.00031998 & 1.00001293 & 1 \\
				\(p_{9}\) & 2.5 & 2.0096071 & 1.9994719 & 2.00009757 & 2 \\
				\(p_{10}\) & 1.25 & 1.01187191 & 0.999948306 & 1.00000074 & 1 \\
				\(p_{11}\) & 2.5 & 1.92166122 & 1.99779729 & 1.99996503 & 2 \\
				\(p_{12}\) & 1.25 & 1.28010632 & 0.970008073 & 1.0006003 & 1 \\
				\(p_{13}\) & 1.25 & 1.24789258 & 1.02128098 & 1.00046207 & 1 \\
				\(p_{14}\) & 1.25 & 1.03907485 & 1.00054265 & 1.00006644 & 1 \\
				\(p_{15}\) & 2.5 & 2.02375596 & 2.00025627 & 2.00042393 & 2 \\
				\(p_{16}\) & 1.25 & 0.95682198 & 0.999214557 & 0.999924966 & 1 \\
				\(p_{17}\) & 2.5 & 2.03220726 & 2.00004683 & 2.00005304 & 2 \\
				\(p_{18}\) & 1.25 & 1.30796856 & 1.0213542 & 1.00054559 & 1 \\
				\(p_{19}\) & 0.125 & 0.0835616326 & 0.099729313 & 0.100006054 & 0.1 \\
				\(p_{20}\) & 1.25 & 0.937925787 & 1.00009982 & 1.00017143 & 1 \\
				\(p_{21}\) & 0.125 & 0.0805224159 & 0.0997250342 & 0.0999962253 & 0.1 \\
				\(p_{22}\) & 0.125 & 0.0523304684 & 0.0958432134 & 0.0999950946 & 0.1 \\
				\(p_{23}\) & 1.25 & 0.797973803 & 0.996369022 & 0.999967589 & 1 \\
				\(p_{24}\) & 0.125 & 0.0511887148 & 0.0961161063 & 0.0999976432 & 0.1 \\
				\(p_{25}\) & 0.125 & 0.0969006972 & 0.099410771 & 0.0999977417 & 0.1 \\
				\(p_{26}\) & 1.25 & 0.958029225 & 1.00100699 & 1.00005045 & 1 \\
				\(p_{27}\) & 0.125 & 0.0984874482 & 0.0993193309 & 0.0999939702 & 0.1 \\
				\(p_{28}\) & 1.25 & 0.949328558 & 1.00095809 & 0.999982293 & 1 \\
				\(p_{29}\) & 1.25 & 1.17061358 & 1.00022773 & 0.999773012 & 1 \\
				\(p_{30}\) & 1.25 & 1.44501769 & 0.991610326 & 0.999712329 & 1 \\
				\(p_{31}\) & 1.25 & 1.00314754 & 1.00046588 & 1.00004543 & 1 \\
				\(p_{32}\) & 1.25 & 1.13434669 & 1.00318027 & 0.999760709 & 1 \\
				\(p_{33}\) & 1.25 & 1.11995395 & 0.995898142 & 0.999374336 & 1 \\
				\(p_{34}\) & 1.25 & 1.07549336 & 1.00004426 & 0.999912615 & 1 \\
				\(p_{35}\) & 1.25 & 1.13916049 & 1.00206694 & 0.999828481 & 1 \\
				\(p_{36}\) & 1.25 & 1.02150821 & 0.999322023 & 0.999867458 & 1 \\
				$\alpha$ & & 3.31262929 & 0.0663801233 & \num{1.91026747e-07} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 16 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points. Regularization parameter \(\alpha\) was determined using \eqref{eq:alphaformula} where \(C = 0.009\) and \(\gamma = 2\).}
\label{tab:tsmn01}
\end{table}


==> table/tsmn_no_noise_16ds_21.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSS}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{4}$ & $\vecu_{7}$ & $\vecu$ \\ \midrule
			\(p_{1}\) & 1.25 & 1.25512524 & 0.927122051 & 1.00085724 & 1 \\
			\(p_{2}\) & 1.25 & 0.999862712 & 1.00002606 & 1.00000674 & 1 \\
			\(p_{3}\) & 2.5 & 1.97178799 & 1.99991702 & 1.99991175 & 2 \\
			\(p_{4}\) & 1.25 & 0.990143871 & 0.999896404 & 0.999994678 & 1 \\
			\(p_{5}\) & 2.5 & 1.95853912 & 1.99985784 & 1.9999685 & 2 \\
			\(p_{6}\) & 1.25 & 1.25267822 & 0.92718216 & 1.00085391 & 1 \\
			\(p_{7}\) & 1.25 & 1.29546916 & 0.921503261 & 1.00050106 & 1 \\
			\(p_{8}\) & 1.25 & 0.998113434 & 1.0000227 & 1.00001141 & 1 \\
			\(p_{9}\) & 2.5 & 1.9878538 & 2.00007904 & 2.00010144 & 2 \\
			\(p_{10}\) & 1.25 & 1.01372789 & 0.99997927 & 1.00000172 & 1 \\
			\(p_{11}\) & 2.5 & 1.99703695 & 1.99988845 & 1.99997249 & 2 \\
			\(p_{12}\) & 1.25 & 1.29427485 & 0.921414646 & 1.00050365 & 1 \\
			\(p_{13}\) & 1.25 & 1.26093202 & 0.93060889 & 1.00051206 & 1 \\
			\(p_{14}\) & 1.25 & 1.01330944 & 0.999998143 & 1.00006177 & 1 \\
			\(p_{15}\) & 2.5 & 1.94676303 & 1.99988776 & 2.00039646 & 2 \\
			\(p_{16}\) & 1.25 & 0.985547194 & 1.00000026 & 0.999930404 & 1 \\
			\(p_{17}\) & 2.5 & 1.97327136 & 2.00003146 & 2.00004305 & 2 \\
			\(p_{18}\) & 1.25 & 1.27616544 & 0.930140952 & 1.00058938 & 1 \\
			\(p_{19}\) & 0.125 & 0.0843118088 & 0.0997088575 & 0.100006441 & 0.1 \\
			\(p_{20}\) & 1.25 & 0.981821731 & 1.00011001 & 1.00013735 & 1 \\
			\(p_{21}\) & 0.125 & 0.0776212027 & 0.0996417541 & 0.0999985603 & 0.1 \\
			\(p_{22}\) & 0.125 & 0.086556167 & 0.0999725968 & 0.0999951983 & 0.1 \\
			\(p_{23}\) & 1.25 & 0.956213743 & 0.999841926 & 0.99996116 & 1 \\
			\(p_{24}\) & 0.125 & 0.0854886179 & 0.0999785954 & 0.09999813 & 0.1 \\
			\(p_{25}\) & 0.125 & 0.0852485971 & 0.0999880247 & 0.0999983637 & 0.1 \\
			\(p_{26}\) & 1.25 & 0.984253636 & 0.999697311 & 1.00007222 & 1 \\
			\(p_{27}\) & 0.125 & 0.0822077677 & 0.0999874859 & 0.0999931404 & 0.1 \\
			\(p_{28}\) & 1.25 & 0.907849342 & 0.999259411 & 0.999987714 & 1 \\
			\(p_{29}\) & 1.25 & 1.10586514 & 0.999880724 & 0.99978328 & 1 \\
			\(p_{30}\) & 1.25 & 1.34338671 & 1.00104412 & 0.999682621 & 1 \\
			\(p_{31}\) & 1.25 & 1.00716795 & 0.999721591 & 1.0000418 & 1 \\
			\(p_{32}\) & 1.25 & 1.09480976 & 0.999454313 & 0.999775109 & 1 \\
			\(p_{33}\) & 1.25 & 0.986460944 & 0.999899864 & 0.999384976 & 1 \\
			\(p_{34}\) & 1.25 & 0.991171566 & 0.999655209 & 0.999901482 & 1 \\
			\(p_{35}\) & 1.25 & 1.04745953 & 0.99934233 & 0.999822786 & 1 \\
			\(p_{36}\) & 1.25 & 0.974965866 & 1.00029979 & 0.99987451 & 1 \\
			$\alpha$ & & 2.01103137 & 0.00931903131 & \num{2.68809336e-08} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{With 16 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 6.0\), which give us 20 data vectors per data set. We found \(\alpha\) as a function of the residual where \(C = 0.005\) and \(S = 2\). }
\label{tab:tsmn01_21}
\end{table}


==> table/tsmn_noise_05ds_0p01.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{4}$ & $\vecu_{7}$ & $\vecu$ \\ \midrule
		\(p_{1}\) & 1.25 & 0.789042988 & 1.04087601 & 1.04097484 & 1 \\
		\(p_{2}\) & 1.25 & 0.993026319 & 1.03234173 & 1.03197336 & 1 \\
		\(p_{3}\) & 2.5 & 1.98862328 & 1.93300927 & 1.93278995 & 2 \\
		\(p_{4}\) & 1.25 & 1.04623302 & 1.00235358 & 1.0041178 & 1 \\
		\(p_{5}\) & 2.5 & 2.1145315 & 2.00368165 & 2.00338784 & 2 \\
		\(p_{6}\) & 1.25 & 0.789083544 & 1.03966884 & 1.03957014 & 1 \\
		\(p_{7}\) & 1.25 & 0.824964803 & 0.988018736 & 0.98673887 & 1 \\
		\(p_{8}\) & 1.25 & 0.919250389 & 0.99326011 & 0.993246801 & 1 \\
		\(p_{9}\) & 2.5 & 2.02745523 & 2.02958003 & 2.02961926 & 2 \\
		\(p_{10}\) & 1.25 & 1.00996579 & 0.999024142 & 0.998881252 & 1 \\
		\(p_{11}\) & 2.5 & 1.91115438 & 1.9902297 & 1.99022601 & 2 \\
		\(p_{12}\) & 1.25 & 0.816637416 & 0.986669984 & 0.987960306 & 1 \\
		\(p_{13}\) & 1.25 & 0.707889111 & 0.459159742 & 0.469475449 & 1 \\
		\(p_{14}\) & 1.25 & 0.894428974 & 1.01709936 & 1.01838585 & 1 \\
		\(p_{15}\) & 2.5 & 2.20122811 & 1.8080775 & 1.80832768 & 2 \\
		\(p_{16}\) & 1.25 & 1.25306624 & 0.954100642 & 0.946776478 & 1 \\
		\(p_{17}\) & 2.5 & 1.74485706 & 2.15385916 & 2.15266302 & 2 \\
		\(p_{18}\) & 1.25 & 0.583645574 & 0.505583645 & 0.495461991 & 1 \\
		\(p_{19}\) & 0.125 & 0.0886884376 & 0.0997886533 & 0.100295276 & 0.1 \\
		\(p_{20}\) & 1.25 & 0.956177019 & 0.997899719 & 0.998500125 & 1 \\
		\(p_{21}\) & 0.125 & 0.0905840768 & 0.0999087146 & 0.100344901 & 0.1 \\
		\(p_{22}\) & 0.125 & 0.0907166241 & 0.0990826121 & 0.0992177486 & 0.1 \\
		\(p_{23}\) & 1.25 & 1.01870288 & 0.998595576 & 0.998033557 & 1 \\
		\(p_{24}\) & 0.125 & 0.0886090313 & 0.0991564505 & 0.0992812541 & 0.1 \\
		\(p_{25}\) & 0.125 & 0.0963271698 & 0.102086585 & 0.100910182 & 0.1 \\
		\(p_{26}\) & 1.25 & 0.985426128 & 0.978906303 & 0.977708668 & 1 \\
		\(p_{27}\) & 0.125 & 0.0961414889 & 0.103664063 & 0.102364328 & 0.1 \\
		\(p_{28}\) & 1.25 & 0.994565032 & 1.00654159 & 1.00938623 & 1 \\
		\(p_{29}\) & 1.25 & 1.26577676 & 0.966400723 & 0.967307622 & 1 \\
		\(p_{30}\) & 1.25 & 1.38032993 & 0.904214109 & 0.904649214 & 1 \\
		\(p_{31}\) & 1.25 & 1.04786493 & 1.01638723 & 1.01567894 & 1 \\
		\(p_{32}\) & 1.25 & 1.19024051 & 0.955823738 & 0.955515177 & 1 \\
		\(p_{33}\) & 1.25 & 1.06494286 & 0.845880507 & 0.845803197 & 1 \\
		\(p_{34}\) & 1.25 & 1.11411486 & 0.990735244 & 0.988494903 & 1 \\
		\(p_{35}\) & 1.25 & 1.26031189 & 0.983263118 & 0.983132056 & 1 \\
		\(p_{36}\) & 1.25 & 1.02583522 & 0.976956736 & 0.977586394 & 1 \\
		$\alpha$ & & 1.8478498 & 0.00232630507 & \num{1E6} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 1\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points.}\label{tab:tsmn_noise_01}
\end{table}


==> table/tsmn_noise_05ds_0p03.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{5}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 1.25 & 0.836336411 & 1.22164808 & 1 \\
				\(p_{2}\) & 1.25 & 0.923863675 & 0.910236274 & 1 \\
				\(p_{3}\) & 2.5 & 2.25014245 & 2.29944049 & 2 \\
				\(p_{4}\) & 1.25 & 1.00463777 & 1.01222856 & 1 \\
				\(p_{5}\) & 2.5 & 1.98776216 & 1.99398704 & 2 \\
				\(p_{6}\) & 1.25 & 0.835989847 & 1.22186735 & 1 \\
				\(p_{7}\) & 1.25 & 0.880298886 & 0.899171499 & 1 \\
				\(p_{8}\) & 1.25 & 0.903396025 & 0.965961263 & 1 \\
				\(p_{9}\) & 2.5 & 2.06301724 & 2.10559939 & 2 \\
				\(p_{10}\) & 1.25 & 1.00737929 & 0.99779859 & 1 \\
				\(p_{11}\) & 2.5 & 1.78598163 & 1.93183892 & 2 \\
				\(p_{12}\) & 1.25 & 0.861206601 & 0.894629405 & 1 \\
				\(p_{13}\) & 1.25 & 0.775511645 & 1.03551575 & 1 \\
				\(p_{14}\) & 1.25 & 0.998741283 & 1.02928328 & 1 \\
				\(p_{15}\) & 2.5 & 2.00159064 & 1.93659065 & 2 \\
				\(p_{16}\) & 1.25 & 0.906726796 & 0.936961938 & 1 \\
				\(p_{17}\) & 2.5 & 1.91148849 & 2.16269593 & 2 \\
				\(p_{18}\) & 1.25 & 0.803302684 & 1.10285114 & 1 \\
				\(p_{19}\) & 0.125 & 0.0982782757 & 0.0987103061 & 0.1 \\
				\(p_{20}\) & 1.25 & 1.02863726 & 1.06692718 & 1 \\
				\(p_{21}\) & 0.125 & 0.0966970444 & 0.0950209661 & 0.1 \\
				\(p_{22}\) & 0.125 & 0.112588901 & 0.109833999 & 0.1 \\
				\(p_{23}\) & 1.25 & 0.976819907 & 0.970522587 & 1 \\
				\(p_{24}\) & 0.125 & 0.113772022 & 0.111934222 & 0.1 \\
				\(p_{25}\) & 0.125 & 0.0959789043 & 0.0973510415 & 0.1 \\
				\(p_{26}\) & 1.25 & 0.948764487 & 0.956708649 & 1 \\
				\(p_{27}\) & 0.125 & 0.0977163991 & 0.100637264 & 0.1 \\
				\(p_{28}\) & 1.25 & 0.993411766 & 1.00423057 & 1 \\
				\(p_{29}\) & 1.25 & 1.18330966 & 1.10321248 & 1 \\
				\(p_{30}\) & 1.25 & 1.40360268 & 1.19869956 & 1 \\
				\(p_{31}\) & 1.25 & 1.03751688 & 1.0422222 & 1 \\
				\(p_{32}\) & 1.25 & 1.10627543 & 1.04779353 & 1 \\
				\(p_{33}\) & 1.25 & 1.09918042 & 0.984786136 & 1 \\
				\(p_{34}\) & 1.25 & 1.12389178 & 1.0784948 & 1 \\
				\(p_{35}\) & 1.25 & 1.20869341 & 1.11237206 & 1 \\
				\(p_{36}\) & 1.25 & 1.03140497 & 1.0045884 & 1 \\
				$\alpha$ & & 0.398107171 & \num{1E6} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 3\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points.}
\label{tab:tsmn_noise_03}
\end{table}


==> table/tsmn_noise_05ds_0p05.tex <==
\begin{table}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSc}
		\toprule
		$\vecu$ & $\vecu_{0}$ & $\vecu_{2}$ & $\vecu_{5}$ & $\vecu$ \\ \midrule
				\(p_{1}\) & 1.25 & 0.936203419 & 0.936105174 & 1 \\
				\(p_{2}\) & 1.25 & 0.944607209 & 0.945127102 & 1 \\
				\(p_{3}\) & 2.5 & 2.0641821 & 2.06438867 & 2 \\
				\(p_{4}\) & 1.25 & 1.13617851 & 1.13488149 & 1 \\
				\(p_{5}\) & 2.5 & 2.33023755 & 2.33025791 & 2 \\
				\(p_{6}\) & 1.25 & 0.931285379 & 0.930996893 & 1 \\
				\(p_{7}\) & 1.25 & 0.867591965 & 0.868217193 & 1 \\
				\(p_{8}\) & 1.25 & 0.852488669 & 0.850891068 & 1 \\
				\(p_{9}\) & 2.5 & 2.13988987 & 2.14002749 & 2 \\
				\(p_{10}\) & 1.25 & 1.04382816 & 1.04517098 & 1 \\
				\(p_{11}\) & 2.5 & 2.16858568 & 2.16928963 & 2 \\
				\(p_{12}\) & 1.25 & 0.871242913 & 0.871135067 & 1 \\
				\(p_{13}\) & 1.25 & 0.763352238 & 0.764159258 & 1 \\
				\(p_{14}\) & 1.25 & 0.910831108 & 0.910979551 & 1 \\
				\(p_{15}\) & 2.5 & 2.28357607 & 2.28354628 & 2 \\
				\(p_{16}\) & 1.25 & 1.29385402 & 1.2935173 & 1 \\
				\(p_{17}\) & 2.5 & 1.88827308 & 1.88834872 & 2 \\
				\(p_{18}\) & 1.25 & 0.569715984 & 0.568710035 & 1 \\
				\(p_{19}\) & 0.125 & 0.0775256688 & 0.0700250919 & 0.1 \\
				\(p_{20}\) & 1.25 & 1.00831334 & 1.00806498 & 1 \\
				\(p_{21}\) & 0.125 & 0.0756479377 & 0.0685355699 & 0.1 \\
				\(p_{22}\) & 0.125 & 0.0172301513 & 0.0348019282 & 0.1 \\
				\(p_{23}\) & 1.25 & 1.31492384 & 1.31534118 & 1 \\
				\(p_{24}\) & 0.125 & 0.0140875938 & 0.0290542096 & 0.1 \\
				\(p_{25}\) & 0.125 & 0.118236483 & 0.117676579 & 0.1 \\
				\(p_{26}\) & 1.25 & 0.899598233 & 0.899770838 & 1 \\
				\(p_{27}\) & 0.125 & 0.132363964 & 0.132992632 & 0.1 \\
				\(p_{28}\) & 1.25 & 0.926567325 & 0.923786316 & 1 \\
				\(p_{29}\) & 1.25 & 1.27854338 & 1.27819705 & 1 \\
				\(p_{30}\) & 1.25 & 1.27716944 & 1.27681757 & 1 \\
				\(p_{31}\) & 1.25 & 0.996671275 & 0.999608566 & 1 \\
				\(p_{32}\) & 1.25 & 1.25748571 & 1.25701102 & 1 \\
				\(p_{33}\) & 1.25 & 1.14858208 & 1.14899508 & 1 \\
				\(p_{34}\) & 1.25 & 1.02745463 & 1.0266701 & 1 \\
				\(p_{35}\) & 1.25 & 1.19609195 & 1.19671813 & 1 \\
				\(p_{36}\) & 1.25 & 1.00266771 & 1.00231793 & 1 \\
				$\alpha$ & & 89.1250938 & \num{1E6} &  \\
		\bottomrule
	\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters at select iterations, with 5\% noise, 5 data sets, \(t_0 = 0\), \(t_1 = 120\), \(\Delta t = 0.5\), i.e. 240 time points.}
\label{tab:tsmn_noise_05}
\end{table}


==> table/tsmn_num_of_data_pnts.tex <==
\begin{table}
    \sisetup{
	    round-precision = 3,
		tight-spacing = true
	}
\centering
\begin{adjustbox}{clip=false}
	\begin{tabular}{lSSSc}
		\toprule
		$\vecu$ & 1 & 20 &  240 & $\vecu$  \\ \midrule
\(p_{1}\) 			& 	0.939248702 		& 	0.999957777   		& 	0.999985309 	& 	1 \\
\(p_{2}\) 			& 	1.00000107 			& 	0.999973605          & 0.999980727 		& 	1 \\
\(p_{3}\) 			& 	1.99999419 			& 	2.00005281 	        & 	2.00004005 		& 	2 \\
\(p_{4}\) 			& 	0.999936216 		& 	0.999997884          & 0.999999321 		& 	1 \\
\(p_{5}\) 			& 	1.99980444 			& 	1.99999171 	        & 	1.99999485 		& 	2 \\
\(p_{6}\) 			& 	0.939247299 		& 	0.999957854          & 0.999985421 		& 	1 \\
\(p_{7}\) 			& 	1.27876764 			& 	0.999882968          & 0.999940451 		& 	1 \\
\(p_{8}\) 			& 	0.999962629 		& 	1.00005757 	        & 	1.00004606 		& 	1 \\
\(p_{9}\) 			& 	2.00005329 			& 	1.99984909 	        & 	1.99988039 		& 	2 \\
\(p_{10}\) 			& 	1.00000035 			& 	1.0000022 	        & 	1.00000207 		& 	1 \\
\(p_{11}\) 			& 	2.00026421 			& 	2.00012953 	        & 	2.00010423 		& 	2 \\
\(p_{12}\) 			& 	1.27877473 			& 	0.999893086          & 0.999948536 		& 	1 \\
\(p_{13}\) 			& 	1.11704615 			& 	0.999846624          & 1.00007969 		& 	1 \\
\(p_{14}\) 			& 	1.00009858 			& 	0.999963939          & 0.999967429 		& 	1 \\
\(p_{15}\) 			& 	1.99966958 			& 	2.00009842 	        & 	2.00009505 		& 	2 \\
\(p_{16}\) 			& 	0.999828363 		& 	1.00009515 	        & 	1.00008893 				& 	1 \\
\(p_{17}\) 			& 	2.00029273 			& 	1.99983787 	        & 	1.99984595 			& 	2 \\
\(p_{18}\) 			& 	1.11720281 			& 	0.999758607          & 0.999997855 		& 	1 \\
\(p_{19}\) 			& 	0.0796494801		& 	0.0999996257        & 0.100000093 		& 	0.1 \\
\(p_{20}\) 			& 	1.000016 			& 	0.999991121          & 0.999999015 		& 	1 \\
\(p_{21}\) 			& 	0.0796543499		& 	0.100000095          & 0.100000113 		& 	0.1 \\
\(p_{22}\) 			& 	0.116383757 		& 	0.0999966337        & 0.0999967426		& 	0.1 \\
\(p_{23}\) 			& 	0.999985667 		& 	0.999997822          & 0.999994898 		& 	1 \\
\(p_{24}\) 			& 	0.11636584 			& 	0.0999967151        & 0.0999970026		& 	0.1 \\
\(p_{25}\) 			& 	0.116242053 		& 	0.100008936          & 0.10000601 			& 	0.1 \\
\(p_{26}\) 			& 	1.00010004 			& 	0.999989177          & 0.99998832 			& 	1 \\
\(p_{27}\) 			& 	0.116183663 		& 	0.100009706          & 0.100006855 		& 	0.1 \\
\(p_{28}\) 			& 	1.16713983 			& 	0.999989245          & 0.999993564 		& 	1 \\
\(p_{29}\) 			& 	1.01160191 			& 	1.00006756 	        & 	1.00003569 			& 	1 \\
\(p_{30}\) 			& 	1.019334 			& 	1.00017592 	        & 	1.00009755 			& 	1 \\
\(p_{31}\) 			& 	1.17016031 			& 	1.00000211 	        & 	0.999998128 		& 	1 \\
\(p_{32}\) 			& 	1.00849871 			& 	1.00004825 	        & 	1.00003109 			& 	1 \\
\(p_{33}\) 			& 	1.00681577 			& 	1.00013364 	        & 	1.00009864 			& 	1 \\
\(p_{34}\) 			& 	1.17263346 			& 	1.00001861 	        & 	1.00000862 			& 	1 \\
\(p_{35}\) 			& 	1.00920322 			& 	1.00001572 	        & 	1.00000312 			& 	1 \\
\(p_{36}\) 			& 	1.00147431 			& 	0.999987584          & 0.999981958 		& 	1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{The evolution of the parameters as the number of time points increase, from 1 to 240. Where 5 data sets were considered, \(\mathbf{u}_0 = 1.25\mathbf{u} \). In each case regularization parameter \(\alpha\) is chosen near optimally.}
\label{tab:tsmn_num_of_data_pnts}
\end{table}


==> table/tsmn_num_of_id_params.tex <==
\begin{table}
\centering
	\begin{tabular}{cc}
		\toprule
		{Data sets} & {Identifiable parameters} \\ \midrule
		1&18 \\
        2&20 \\
        3&31 \\
        4&31 \\
        5&36 \\
		\bottomrule
	\end{tabular}
\caption{The number of data sets versus the number of identifiable parameters. Gathered from the analysis done in~\cite{identif2}.}
\label{tab:num_of_id_params}
\end{table}

